Intent Graph: Navigating the Analytical Reasoning Space for Exploratory Data Analysis

Exploratory data analysis (EDA) is rarely open-ended in practice: analysts work from high-level domain questions toward the concrete analyses that can answer them, prioritizing directions with domain knowledge and prior hypotheses. Large language models (LLMs) can supply such knowledge, but their responses are unstructured, leaving analysts no way to see what has been explored, what is missing, or why one direction was chosen over another. We present DAG-EDA, a system that lets analysts and an LLM co-navigate the space of possible analyses through two linked structures. An intent graph, governed by a grammar of analytical intent, decomposes an ambiguous natural-language question into progressively concrete analysis tasks, keeping alternative framings open and letting analysts branch, backtrack, and compare paths. A multi-layered knowledge graph externalizes the LLM's domain knowledge, linking domain concepts to the dataset variables that can measure them, so analysts can inspect and contest how their question is grounded in the data. Both graphs are constructed from only the dataset and the analyst's question, and the analyses the analyst reaches are rendered as interactive dashboards. We illustrate the system through a usage scenario and describe a user study design for examining whether the system scaffold analysts' reasoning and navigation.

==> sections/7-grammar.tex <==
\section{Intent Grounding Framework: a formal grammar for analytical reasoning}

\leilani{Open-ended data exploration begins with questions that are often ambiguous and underspecified. There is no evidence that all analytical reasoning follows this process. We need to be more precise.}
Analytical reasoning begins with questions that are often ambiguous and underspecified. "What makes movies successful?" could mean describing revenue distributions, identifying causal factors, comparing genres, or forecasting trends. Before we can leverage domain knowledge (concept layer) or data relationships (data layer) to generate analyses, we must first ground these questions to specific analytical intents.
\leilani{The mantra "seek first to understand before seeking to be understood" comes to mind here. The ultimate goal is to understand what the user is trying to learn through their question. To do this, we try to ground that question in a specific domain context, then try to understand how that domain context may or may not connect to the dataset they shared. Finally, the system needs to communicate its understanding to the user and get their feedback. This is the purpose of the grammar, to externalize the system's reasoning process in a consistent format and to invite the user to express their reasoning process in the same format, with the goal of enabling the user and system to collaboratively develop a shared understanding of the intent behind the analysis question (and if necessary, change the analysis question to better match the user's true intent).}

This section presents a formal grammar for decomposing analytical questions through progressive disambiguation. 
We identify two intertwined types of ambiguity: question framing ambiguity (what analytical relationship to investigate) and concept ambiguity (what concepts mean in terms of data). 
They mutually constrain each other to narrow the space of possible analyses. 
Our grammar defines how questions are structured, what counts as a valid question, and how underspecified questions resolve to executable forms. 
\junran{This section focuses specifically on the intent layer structure and decomposition rules. How the intent grammar integrates with the concept knowledge graph and data causal graph to synthesize concrete analyses is yet to decide.}

\leilani{It worries me that ambiguity is described purely as a means to map the user's intent to data variables. I think what is most important about this project is (a) the system and user collaboratively building a shared analysis intent, using the question as a starting input; and (b) the user and system co-investigating whether the target dataset supports the agreed-upon intent. Data variables only matter in the context of matching the data to the shared representation of analysis intent. The intent is most important. Instead, I would describe disambiguation as an opportunity for the system to express its understanding of the user's analysis intent by demonstrating how the analysis question maps down to concrete, non-ambiguous sub-analyses/sub-tasks. This provides concrete points at which the user can agree or disagree with the system's interpretation.}

% When analysts approach a dataset with questions like ``What makes movies successful?'', they face multiple layers of ambiguity. The term ``successful'' could mean financial revenue, critical ratings, or cultural impact. The question structure itself is underspecified: are they seeking a description, a causal explanation, or a comparison? 
% Even after clarifying these ambiguities, the path from question to concrete data operations remains unclear. 
% Existing text-to-visualization systems often attempt to jump directly from low-level natural language queries to visualizations that achieve corresponding analytical tasks. However, this approach conflates distinct types of ambiguity and misses the opportunity to scaffold the analytical reasoning process itself. We argue that effective analytical tools should make the disambiguation process explicit and interactive, helping analysts refine both what they want to know (intent) and what ambiguous concepts from the question mean (semantics) through a structured dialogue. 
\subsection{Two types of Ambiguity}

\leilani{what are the two types of ambiguity? I would mention them both upfront.}

Concept ambiguity arises when abstract terms in a question lack clear mappings to measurable variables. 
For example,  the term ``successful'' could mean financial revenue, critical ratings, or cultural impact. 
Question framing ambiguity concerns which analytical relationship is being investigated. 
With questions like ``What makes movies successful?'', the question structure itself is underspecified: are they seeking a description, a causal explanation, or a comparison? 

These ambiguities are not independent. They constrain each other bidirectionally that progressively narrows the space of valid analyses. Understanding this constraint propagation is crucial because it explains how partial information from either the question structure or the available concepts can eliminate entire branches of the disambiguation tree. 
Consider a concrete scenario: if "success" is clarified to mean "genre" (a categorical attribute), then the intent "What drives genre?" becomes problematic since genres are not outcomes that are "driven by" other factors in a causal sense. 
This illustrates how concept properties constrain intent space. 
Conversely, if the analyst wants to compare how some quantity differs across categories, the concepts involved must be measurable and comparable along some dimension. 
A single constraint on one dimension can cascade through relationships to eliminate many options in the other dimension, and rapidly converge toward a terminal, executable question. 

\subsection{The Formal Specification}
The grammar defines what analytical intents exist, what parameters they require, how parameters constrain each other, and when an intent becomes executable. Critically, the grammar serves as the control structure for the entire system such that every propagation step, discovery trigger, and constraint check follows grammar rules rather than ad-hoc logic.
The grammar decomposes analytical questions into primitive intents with explicit parameter requirements and dependencies. 
Grammar rules progressively resolve ambiguities through user choices or automated top-K threshold and serve as constraints of the intent propagation mechanism. 
Relevant concepts and data bindings are systematically generated by discovery rules based on intent types. 
Terminal conditions are specified when parameter requirements are satisfied to guarantee excitability. 

\subsubsection{Core Definition}

We identify six primitive intents grounded in data analysis methodology that capture high-level analytical goals: 



\begin{grammar}
  <PrimitiveIntent> ::= DESCRIBE(Variable, Context)
    \alt                 COMPARE(Variable, GroupingFactor, Context)
     \alt                 EXPLAIN(Outcome, Predictors?, Context)
                     \alt  PREDICT(Outcome, Horizon, Context)
                     \alt  EVALUATE(Entity, Criterion, Benchmark, Context)
                     \alt  DISCOVER(Variables, StructureType, Context)
\end{grammar}

\todo{convert the list of intent primitatives in to a table}
\begin{itemize}
    \item DESCRIBE(Variable, Context): Characterize properties of a variable
    \begin{itemize}
        \item Goal: "What are the properties of X?"
        \item Example: "Describe revenue" → histogram, mean, median, range
    \end{itemize}

    \item COMPARE(Variable, GroupingFactor, Context): Contrast across groups
    \begin{itemize}
        \item Goal: "How does X differ across groups?"
        \item Example: "Compare revenue by genre"
    \end{itemize}

    \item EXPLAIN(Outcome, Predictors?, Context): Identify influencing factors
    \begin{itemize}
        \item Goal: "What factors influence Y?"
        \item Example: "What factors influence the revenue?"
    \end{itemize}

    \item PREDICT(Outcome, Condition, Context): Forecast future or counterfactual values
    \begin{itemize}
        \item Goal: "What will Y be?"
        \item Example: "Predict the revenue in year 2026"
    \end{itemize}

    \item EVALUATE(Entity, Criterion, Benchmark, Context): Assess against standard
    \begin{itemize}
        \item Goal: "How well does E perform?"
        \item Example: "Did Oppenheimer meet expectations?"
    \end{itemize}

    \item DISCOVER(Variables, StructureType, Context): Identify latent patterns
    \begin{itemize}
        \item Goal: "What hidden structure exists?"
        \item Example: "Discover audience segments"
    \end{itemize}

\end{itemize}


\leilani{We should have at least one citation for every intent primitive to clarify where they come from in the literature.}

Exploratory terms such as investigate, understand and verify can be modeled as contextual framings of primitive intents. For example, an outlier detected can trigger an EXPLAIN intent that investigate the phenomenon and potential data relationships. 
We recognize one special meta-intent representing underspecified analytical states: 
\begin{grammar}
    <MetaIntent> ::= EXPLORE(Topic, Context)
\end{grammar}
EXPLORE representing the analyst starting fresh from minimal prior knowledge. It requires resolution to primitive intents and decomposes through disambiguation to proceed with the analysis.   



\begin{grammar}
    <AnalyticalQuestion> ::= <Intent>(<Parameters>) \alt <MetaIntent>(<Topic>)

<Intent> ::= <PrimitiveIntent>

<PrimitiveIntent> ::= DESCRIBE(Variable, Context)
                    \alt COMPARE(Variable, GroupingFactor, Context)
                    \alt EXPLAIN(Outcome, Predictors?, Context)
                    \alt PREDICT(Outcome, Condition, Context)
                    \alt EVALUATE(Entity, Criterion, Benchmark, Context)
                    \alt DISCOVER(Variables, StructureType, Context)

<MetaIntent> ::= EXPLORE(Topic, Context)


<Decomposition> ::= <ConceptClarification>
                  \alt <IntentRefinement>
                  \alt <RelationshipSelection>
                  \alt <ParameterSpecification>

<ConceptClarification> ::= AbstractConcept → {ConcreteInterpretation}+
  Example: "success" → {revenue | ratings | awards}

<IntentRefinement> ::= MetaIntent → {PrimitiveIntent}+
  Example: EXPLORE(revenue) → {DESCRIBE | EXPLAIN | COMPARE | PREDICT}

<RelationshipSelection> ::= Intent + Concepts → {Relationship}+
  Example: EXPLAIN(Outcome) → {CAUSATION | CORRELATION}

<TerminalQuestion> ::= <Intent> × <Relationship> × <ConceptBindings> × <Operations>
  where all concepts have data mappings
  and all constraints are satisfied
\end{grammar}

The grammar enforces constraints between the layers of the graph. 
Question frame constrains the valid relationship types between the concept variables in the KG and CG. Concept variable types such as outcome and entity constrain the available relationship types. 

Questions are decomposed through progressive disambiguation including concept clarification and intent frame refinement. 

\subsubsection{Parameter States Definitions}
The grammar defines a formal state machine for each intent parameters. Intent parameters evolve through the following four states:
\begin{itemize}
    \item UNDERSPECIFIED: The parameter has not been explored yet, and no candidates have been discovered
    \item AMBIGUOUS: The parameter has multiple viable candidates, and the user must choose the candidate
    \item PARTIAL: A concept has been selected but hasn't been mapped to actual data yet
    \item GROUNDED: The parameter is fully bound, i.e., both a concept and specific data variable(s) have been selected
\end{itemize}

\leilani{These levels are great! We have talked before about allowing for ambiguity when it's not possible to fully ground the intent in the provided dataset. This should be a satisfactory scenario, since one of our goals is to provide a shared, agreed-upon representation between user and system, and the representation does not need to be fully grounded in the data to be useful in this respect. Another goal is to determine if the dataset is appropriate for answering the question. If we cannot fully ground the corresponding intent in the dataset, then we have detected a mismatch between the dataset and question, which is a good outcome as well.}

The grammar also defines legal transitions between states. For example, you can go from UNDERSPECIFIED to AMBIGUOUS through discovery, or from AMBIGUOUS to GROUNDED through user selection, but you can't jump directly from UNDERSPECIFIED to GROUNDED without discovering candidates first.

\subsubsection{Dependency Rules}
Dependency rules are critical for progressive disambiguation of intent parameters. Each intent explicitly defines dependency relationships between its parameters. Specifically, the grammar defines the following relationships:
\begin{itemize}
    \item depends\_on
    \item independent
\end{itemize}
As an example, in the EXPLAIN intent state, the predictors parameter depends on the outcome parameter. This relationship would be specified via a depends\_on relationship between the two parameters. This relationship means that we cannot discover predictor candidates until the outcome is grounded, and the specific outcome selected determines which predictor variables are relevant. If the outcome were to change, the predictor candidates must be re-discovered.

\subsubsection{Discovery Rules}
Discovery rules define what kind of candidates should be generated for each parameter based on context. These are intent-specific and parameter-sensitive. In particular, discovery rules act as search filters - they tell the system what to look for in the knowledge graph when generating candidates.
\todo{add more detail here?}

\subsubsection{Propagation Rules}
Propagation rules define how binding one parameter should trigger discovery or updates in other parameters. For example, changing the outcome parameter from UNDERSPECIFIED to GROUNDED for the EXPLAIN intent should trigger discovery for the predictors parameter. This action is specified in a propagation rule.

\subsubsection{Terminal Conditions}
Terminal conditions are boolean formulas that determine when an intent is ready to generate operations. Each intent defines a terminal condition that specifies when that intent is fully disambiguated. For example, the terminal condition for the EXPLAIN intent can be described as:
\begin{itemize}
    \item The outcome parameter is in GROUNDED state, AND
    \item Either the predictors parameter is in GROUNDED state, OR the system can automatically discover predictors from the Knowledge Graph
\end{itemize}

Logically, this translates to \texttt{outcome.state == GROUNDED $\land$ (predictors.state == GROUNDED $\lor$ auto\_discover(predictors))}.

Terminal conditions serve to formally guarantee that all constraints on parameter states are satisfied before analysis can proceed.

\leilani{I think we will want to be careful about how we discuss constraints, propagation rules, and terminal conditions. Since the goal is not necessarily to always produce fully-grounded intents (fully grounded in the dataset, I mean), we may want to phrase this as mechanisms we need to do a best-effort grounding of the user's question within a corresponding analysis intent. If possible, we will fully ground the intent in the relevant domain context and provided dataset, but we may only be able to do domain grounding if the dataset is incompatible; figuring this out is one of our design goals.}

\subsubsection{Intent Relationship Rules}
Relationship rules define valid ways that intents can compose, refine, or contextualize each other. The grammar specifies the following relationships between intents:
\begin{itemize}
    \item DECOMPOSES\_TO: A meta-intent with \texttt{terminal\_condition = false} must decompose into one or more primitive intents. The meta-intent represents an underspecified question that must be refined into a specific analytical approach. After decomposition, the meta-intent transitions to DECOMPOSED state and remains in the graph as provenance.
    \begin{itemize}
        \item Applied To: EXPLORE $\rightarrow$ \{EXPLAIN, DESCRIBE, COMPARE, PREDICT, EVALUATE, DISCOVER\}
    \end{itemize}

    \item REFINES\_TO: When a terminal primitive intent reveals structure that warrants deeper investigation, it can refine to another intent focused on that structure. This is a drill-down relationship, i.e., going from broad to specific.

    \item COMPOSES\_TO: When multiple terminal primitive intents share structural similarity, they may compose into a meta-analysis. This is a synthesis relationship, i.e., combining separate analyses to see cross-cutting patterns.

    \item CONTEXTUALIZES\_WITH: An analytical intent may pair with a descriptive intent to provide interpretive context. This is a supporting relationship, i.e., one intent aids interpretation of another without being strictly necessary.
\end{itemize}

Each relationship type has the following:
\begin{itemize}
    \item A condition that must hold for it to be valid
    \item A specification of whether it's mandatory or optional
    \item A description of how intent states change when the relationship is formed
    \item Metadata about why the relationship was created (for user transparency)
\end{itemize}

\subsubsection{Summary}
Together, the aforementioned components work together to define a formal grammar for analytical reasoning, with the goal of transforming ambiguous NL queries into structured analytical intents. Additionally, the grammar serves as executable specification - a precise, unambiguous description of how analytical reasoning should work in the system. This makes the system's behavior predictable and auditable. However, the grammar doesn't implement anything, rather it defines what correct implementation looks like. 

\subsection{Grammar Processor}
The Grammar Processor is the rule enforcement engine. It reads the formal grammar specification and ensures that everything happening in the KG follows the rules. In particular, we use the formal grammar specification as a basis for the grammar parser, which we implemented in Python, using the libraries \texttt{Pydantic} for typed constraint validation and \texttt{Experta} for rule-based inference.

\leilani{We may want to clarify what we mean by rules at a high level. In general, rules to enforce what? That the system's interpretation of the user's intent is as fully domain grounded and data grounded as possible? To restrict how the LLM is allowed to ground the user's analysis question such that it makes sense with the domain and the data?}

\subsubsection{Validation}
We represent each primitive intent and its component parameters using \texttt{Pydantic} data models. Each primitive intent is represented as a strongly typed field, with further constraints including cardinality, admissible data types, and required/optional fields. Representing intents in this way enables us to:
\begin{itemize}
    \item Enforce correctness of analytical states, specifically ensuring that malformed intent instantiations (for example, those that violate type or cardinality constraints) are immediately rejected.
    \item Parameter states (UNDERSPECIFIED, GROUNDED, AMBIGUOUS, and PARTIAL) are explicitly defined, thus providing support for progressive intent grounding.
    \item Allowed relationships within intent parameters and between intents are explicitly defined, enabling early pruning of certain rule-violating analytical paths.
\end{itemize}
Intent nodes can be specified using any data serialization format; in this paper, we use JSON. These schemas are loaded into and validated by the \texttt{Pydantic} models, and these models are used henceforth in discovery.

\subsubsection{Terminal Condition Checking}
Given an intent node, we also wish to evaluate whether it's ready to generate operations. To do so, the \texttt{Pydantic} specification also includes the logical statement evaluating whether or not the node is terminal based on the terminal condition formula described in the grammar.

\subsubsection{Constraint Propagation}
When a parameter gets bound, the grammar processor:
\begin{itemize}
    \item Looks up propagation rules from grammar (e.g., "when outcome is grounded in EXPLAIN, discover predictors")
    \item Identifies which other parameters are affected
    \item Triggers appropriate discovery processes
    \item Updates parameter states based on discovery results
\end{itemize}

It also continuously monitors the composition rules, refinement rules, and contextualization rules of each intent to suggest possible relationships that the user has to accept.

We implement this rule system with \texttt{Experta}, a library for creating rule-based expert systems. We define engines for each intent type, which monitor for changes in parameter states and apply grammar rules to suggest relationships, derive new facts, enforce dependencies, and/or trigger discovery actions.

Overall, we have the following system:
\textbf{Input:} Grammar specification (formal rules), KG intent nodes (current state)
\textbf{Process:} Pattern matching, predicate evaluation, rule application
\textbf{Output:} Validation results, terminal status, triggered propagations, relationship suggestions

\subsubsection{Overall Workflow}

As an example workflow, consider the aforementioned question "What makes movies successful?". Suppose we tie the output parameter to the "Worldwide\_Gross" attribute in our dataset.
\begin{enumerate}
    \item User binds outcome parameter to "Worldwide\_Gross"
    \item Validator checks: "Is Worldwide\_Gross NUMERICAL?" $\rightarrow$ Yes, valid
    \item Grammar Processor finds rule: "outcome grounded $\rightarrow$ discover predictors"
    \item Grammar Processor triggers: KG Manager to run predictor discovery
    \item Grammar Processor evaluates: predictor candidates found, so state = AMBIGUOUS
    \item Grammar Processor checks terminal: outcome=GROUNDED but predictors=AMBIGUOUS $\rightarrow$ Not terminal yet
\end{enumerate}

Generalizing this, we have:
\begin{enumerate}
    \item Initialize intent parameters in UNDERSPECIFIED state
    \item Accept user inputs / concept disambiguations
    \item Validate intent nodes using Pydantic schemas
    \item Input facts into Experta engine
    \item Apply inference rules to suggest relationships, derive new facts, refine intents, and/or trigger discovery actions 
    \item Repeat until terminal conditions are satisfied
\end{enumerate}

With this, we have implemented the rule enforcement engine that validates and processes LLM or user-outputted intent nodes purely deterministically, in order to ensure that they are not violating constraints formally defined in the grammar specification as well as support intent propagation.

\leilani{I think it's fine to write at this level of detail for now, but I suspect we will want to condense things later and make explanatory figures.}

\subsubsection{Integration with Other Layers}



\todo{integration with other layers. still trying to figure this out}

\subsection{Supporting various modality as the terminal node execution}

The current system instantiates terminal nodes as dashboard specification templates, where we map grounded parameters to visual encodings via intent-typed visualization combinations. 
However, the grammar-based intent representation is deliberately output-format-neutral. 
The grounding states, dependency structure, and parameter types encoded in each terminal node constitute a sufficient specification for a range of execution targets. A terminal EXPLAIN node whose outcome and predictors are fully grounded could equally drive a computational notebook containing a regression script, with parameter bindings surfaced as editable variables rather than visual encodings. 
Further, with composable components from Engraft~\cite{engraft}, individual terminal node notebooks can be merged and integrated recursively to mirror the intent graph traversal and execution provonance, where the unified analytical environment's topology reflects the user's exploration path.

More ambitiously, the Boba multiverse specification format!\cite{boba} offers a natural fit: grounded parameters define the analysis decisions that are in scope, while candidates excluded during progressive disambiguation provide a grammar-derived rationale for what the multiverse need not enumerate, which provides a principled boundary that prior multiverse tools require analysts to specify manually. 

Each of these modalities represents a distinct analytical stance, for statisctical, exploratory, and conformatory. 
In this way, the grammar is extensible to low-level execution machinery that prior research established, rather than re-solving those problems from scratch. 
